Virtual Coordinate Backtracking for Void Traversal in Geographic Routing

Geographical routing protocols have several desirable features for use in ad hoc and sensor networks but are susceptible to voids and localization errors. Virtual coordinate systems are an alternative solution to geographically based routing protocols that works by overlaying a coordinate system on the sensors relative to well chosen reference points. VC is resilient to localization errors; however, we show that it is vulnerable to different forms of the void problem and have no viable complementary approach to overcome them. Specifically, we show that there are instances when packets reach nodes with no viable next hop nodes in the forwarding set. In addition, it is possible for nodes with the same coordinates to arise at different points in the network in the presence of voids. This paper identifies and analyzes these problems. It also compares several existing routing protocols based on Virtual Coordinate systems. Finally, it presents a new routing algorithm that uses backtracking to overcome voids to achieve high connectivity in the greedy phase, higher overall path quality and more resilience to localization errors. We show these properties using extensive simulation analysis.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we first demonstrate problems that arise with Virtual
Coordinate based routing and show that contrary to published
conclusions, it is quite vulnerable to voids that arise during greedy
operation.  More specifically, we identify the expanded VC Zone
problem, where nodes of equal VC coordinates span a multiple hop zone.
We also identify the disconnected VC zone problem where nodes sharing
the same VC value occur in geographically disparate locations.
 We show experimentally that these problems have a
considerable effect on reachability provided by VCS algorithms.

The second contribution of the paper is to present a hybrid routing
protocol that replaces the traditional face routing phase used for
void traversal in geographic routing protocols with one based on
virtual coordinates.  We use a simple dimension by dimension
hueristic with backracking along the same dimension as an example of
this type of approach.  We show that the resulting algorithm
significantly outperforms GPSR and BVR in terms of reachability and
path quality.  It is also significantly more resilient to
localization errors, especially those that affect the perimeter
routing phase of the algorithm. Nevertheless, we believe that
improved hueristics in the void traversal phase are still possible.
This is a topic of our future research.


==> introduction.tex <==
\section{Introduction}

\label{sec:introduction}

Traditional ad hoc routing protocols (e.g., AODV~\cite{paper:aodv}),
are not a good fit for Wireless Sensor Networks (WSN) for the
following reasons.  WSNS often require data dissemination patterns
that are not efficiently mapped to the unicast connections assumed
by ad hoc protocols.  Further, nodes need to maintain routing state
specific to destinations of active routes; this state may become
invalid due to changes that are not near to the node.  Finally,
because of the need to maintain non-local state, this approach
requires that the nodes have globally unique identifiers.  As a
result, this approach is not ideal for WSNs which favor routing
protocols that support data-centric operation (e.g., global
identifiers not necessary), localized interactions (e.g.,
maintaining only local state) and supporting arbitrary data-driven
dissemination with in-network processing.

In contrast to traditional ad hoc protocols, Geographical routing
algorithms~\cite{paper:gfg,paper:gpsr,paper:gcrp,paper:practical_gr},
provides attractive properties for WSNs.  In these algorithms, nodes
exchange location information with their neighbors. Packets
addressed to a destination must provide its location.  At every
intermediate hop, the subset of the neighbors that are closer to the
destination is called the forwarding set.  Routing simply forwards a
packet to one of the nodes in the forwarding set.  This process is
repeated greedily until the packet reaches the destination.  Thus,
interactions are localized to location exchange with direct
neighbors and there is no need for global identifiers.

Geographical routing protocols suffer from significant problems
under realistic operation.  First, voids -- intermediate nodes whose
forwarding set (FS) relative to a destination is empty -- can cause
the greedy algorithm to
fail~\cite{paper:gfg,paper:gpsr,paper:bphole,paper:gcrp}. Voids
require a somewhat complex and inefficient complementary perimeter
routing algorithm that is invoked when they are
encountered~\cite{paper:practical_gr}. Moreover, geographic routing
has been shown to be sensitive to localization
errors~\cite{paper:errorgf}, especially in the perimeter routing
phase~\cite{paper:practical_gr,paper:errorfr}; such errors can cause
routing anomalies ranging from suboptimal paths to loops and failure
to deliver packets. Making geographic routing practical is
difficult~\cite{paper:practical_gr}.

Routing based on Virtual Coordinate Systems (VCS) has been recently
proposed~\cite{paper:vcembed,paper:lcr,paper:vcsim,paper:vcap,paper:bvr}.
A VCS overlays virtual coordinates on the nodes in the network based
on their distance (typically in number of hops) from fixed reference
points; the coordinates are computed via an initialization phase.
These coordinates serve in place of the geographic location for
purposes of Geographic forwarding; that is, in these algorithms the
forwarding set is the set of nodes that are closer (based on different
measures of coordinate distances) to the destination than the current
node. Because it does not require precise location information, VCS is
not sensitive to localization errors.

Further, it is argued that VCS is not susceptible to conventional
voids because the coordinates are based on connectivity and not
physical distance \cite{paper:lcr}.  On the negative side, VCS may
be sensitive to collisions and or signal fading effects in the
initialization phase. Furthermore, the initialization phase requires
a flood from each reference point.

The first contribution of the paper is to identify three problems that
arise in VCS routing.  In practice, the three problems occur in fairly
common situations resulting in VCS failing to deliver packets.  In the
first problem, a set of neighbors are all of equal distance to the
destination and greedy forwarding fails.  In the second problem, we
show that nodes with identical coordinates that are far from each
other may arise in the presence of voids.  In the third problem, a
node is closer than any of its neighbors to a given destination, no
matter how the distance is measured. We analyze the frequency of these
problems using a number of random deployment scenarios of different
densities.

The second contribution of the paper is to propose a hybrid routing
protocol.  The protocol uses Greedy Forwarding (GF)
\cite{paper:gfg,paper:gpsr} because of its superior path quality in
the greedy mode.  When voids are encountered, it switches to a VC
based backup algorithm since, intuitively, VC is more effective in
handling physical voids. However, since VC is susceptible to its own
anomalies related to virtual coordinates, routing may still fail; we
use a simple backtracking algorithm where the packet is forwarded
backwards towards an anchor to address such possibilities.  We show
experimentally that it attains high delivery ratio and tolerates
localization errors better than geographically based protocols.  Our
experiment results also show that for all scenarios we used, the
Hybrid geographic and virtual coordinate Greedy Routing (HGR)
provides a 100\% reachability, and much better path quality than
Greedy Perimeter Stateless Routing (GPSR)
\cite{paper:gfg,paper:gpsr}. The greedy nature of HGR makes its
implementation practical and efficient.


 The remainder of this paper is organized as follows.  Section
 \ref{sec:related} provides an overview of the related works.  After
 analyzing the problems of existing protocols and VCS in section
 \ref{sec:vcsproblems}, we present the design of HGR in section
 \ref{sec:hgr}.  In, Section \ref{sec:experiment} we present an
 experimental study analyzing the different routing protocols.
 Finally, Section \ref{sec:conclusion} presents some concluding
 remarks.


==> related.tex <==
\section{Background and Related Work}
\label{sec:related}

 Shortest Path (SP) routing is a commonly-used for sensor networks.
 In this protocol, data sinks send periodic advertisements that flood
 the network.  As nodes receive the beacon, they set their next hop to
 the neighbor advertising the shortest distance to the sink.  SP can
 provide the optimal path in terms of path length.  However, it is a
 stateful (not stateless) and reactive protocol: for each destination, the forwarding
 path is needed before data transmission can begin.  The storage it
 requires increases with the number of destinations in the network.
 Furthermore, it is vulnerable to mobility or other changes in the
 topology.

  In ad hoc and sensor networks, stateless routing, where the routing
state is independent of the traffic, is desirable.  Geographical
routing protocols with the stateless
property~\cite{paper:gfg,paper:gpsr}; in the base mode, they use GF,
where each node forwards packets to a neighbor that will bring the
packet closest to the destination. Each node tracks only the
location information of its neighbors. The {\em forwarding set} for
a given destination is the subset of neighbors closer to the
destination.  GF proceeds by picking a node from this set, typically
the closest one to the destination.  If the forwarding set is empty,
a {\em void} is encountered.  Typically, a complementary algorithm
is used to traverse the void.  Face routing (or perimeter routing)
is an approach based planar graph theory often used for void
traversal. The general idea in face routing is to attempt to route
around the void using a right hand rule that selects node around the
perimeter of the void (details may be found in the original
paper~\cite{paper:gfg,paper:gpsr}).  Face routing stops when a node
closer to the destination than the void origin is encountered; at
this stage, operation switches back to greedy forwarding.

Since GPS devices are costly, they may not be feasible for sensor
networks; often, localization algorithms are employed that
significantly increase the uncertainty in the location estimate
(e.g.,~\cite{paper:aps,paper:robustloc-mobicom2002}).  Both GF and
face routing are susceptible to localization
errors~~\cite{paper:errorgf,paper:errorfr}. While some approaches to
tolerate location errors have been suggested, in general, this remains
a weakness of this class of protocols. Further, the paths constructed
by face routing are typically not the best path available to cross the
void.  Thus, additional routing protocols have attempted to optimize
the face routing phase of
operation~\cite{paper:gcrp,paper:bphole,paper:glider}.

Kim et al \cite{paper:practical_gr} recognize effects that arise in
practice during geographic routing and suggest a protocol which uses
more control packets to planarize the network. The algorithm requires
more resources and is stateful.

Routing based on a coordinate system was first proposed by Rao et
al~\cite{paper:grnoloc}.  Their algorithm requires a large number of
nodes to serve as virtual coordinate anchors (sufficient to form a
bounding polygon around the remaining sensors).  A large number of
anchor nodes increases the overhead as well as the state maintained by
each node.  The location estimated by the virtual coordinates is used
for geographic routing. Their approach is more accurately described as
a localization mechanism for use in an otherwise geographically based
algorithm.  It is unclear if face routing will be effective with a
coarse-grained location estimate.

Caruso et al recently proposed the Virtual Coordinate assignment
protocol (VCap)~\cite{paper:vcap}; several similar protocols were
proposed by
others~\cite{paper:vcembed,paper:vcsim,paper:lcr,paper:geow/o,paper:bvr}.
In this approach, coordinates are constructed in an initialization
phase relative to a number of reference points. Following this
initialization phase, packets can be routed using the Greedy
Forwarding principles, replacing node location with its coordinates.
The paper uses 3 reference points to assign the virtual coordinates,
constructing a 3-dimensional VCS. The authors identified the {\em VC
Zone} (several nodes assigned to the same virtual coordinates)
problem and provided bounds on its size. (The original research work
on VC Zone can be found in \cite{paper:landmarks,paper:geow/o} with
more details.) The authors do offer a heuristic for situations where
voids are encountered: they suggested a {\em local detour} to
forward packet to some neighbor farther away to destination several
times in hope of reaching some node with a different path to the
destination; this approach may lead to longer paths as packets are
misrouted. The evaluation in the paper shows that VCap performs
worse than GPSR both in delivery ratio and path stretch.


Qing et al proposed a similar protocol to VCap with 4 reference nodes
(4D) each located at a corner for a rectangle area \cite{paper:lcr}.
The authors suggested a backtracking approach to packet delivery when
facing any routing anomalies, which requires each hop in the
forwarding path of each packet to be recorded. The authors did not
analyze either why or when these anomalies happen. Although this
backtracking approach converges, in the worst case, it will go through
all the nodes in the network.

Using Manhattan-style distance (MD) in place of Euclidean distance
(ED) was proposed by Rodrigo et al in BVR\cite{paper:bvr}. On a VCS
with a very high number of reference nodes (typically 10 to 80), BVR
suggested a different backtracking approach to send packets to the
reference node closest to the destination when greedy forwarding
fails. As we show in this paper, neither Manhattan distance or the
one proposed in BVR\cite{paper:bvr} (we called semi-Manhattan
distance) are a good measure of distance compared to a Euclidean
distance. Having that many reference nodes require much more
resources and may also hurt the performance of any practical sensor
networks.


 Papadimitriou and Ratajczak~\cite{paper:gfconjecture}
conjecture that every planar 3-connected graph can be embedded on
the plane so that greedy routing works.  If this conjecture holds,
then for planarized networks, a guaranteed greedy routing may exist.
GEM~\cite{paper:gem} proposed the routing based on a virtual
coordinate system. A virtual polar coordinate space (VPCS) is used
for localizing each node in network. A tree-style overlay is then
used for routing. Using the tree overlay results in poor path
quality.  Since it uses the VPCS to localize the network first, it
tolerates only up to $10\%$ localization error~\cite{paper:gem}.

